Examining the Role of Chloride Ligands on Defect Removal in Imperfectly Attached Semiconductor Nanocrystals for 1D and 2D Attachment Cases

Semiconducting, core-shell nanocrystals (NCs) are promising building blocks for the construction of higher dimensional artificial nanostructures using oriented attachment. However, the assembly and epitaxial attachment steps critical to this construction introduce disorder and defects which inhibit the observation of desirable emergent electronic phenomena. Consequently, understanding defect formation and remediation in these systems as a function of dimensionality is a crucial step to perfecting their synthesis. In this work, we use in situ high resolution transmission electron microscopy to examine the role of chloride ligands as remediator agents for imperfect attachment interfaces between CdSe/CdS core-shell NCs for both 1D and 2D attachment cases. In the 1D case, we find that the presence of chloride additives in imperfectly attached NC dimers can result in defect removal speeds nearly twice as large as those found in their plain, non-chloride treated counterparts. However, when we increased the dimensionality of the system and examined 2D NC arrays, we found no statistically significant difference in attachment interface quality between the chloride and non-chloride treated samples. We propose that this discongruity arises from fundamental differences between 1D and 2D NC attachment and discuss synthetic guidelines to inform future nanomaterial superlattice design.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
